Sum of Consecutive Terms of Pell and Related Sequences

We study new identities related to the sums of adjacent terms in the Pell sequence, defined by $P_{n} := 2P_{n-1}+P_{n-2}$ for $ n\geq 2$ and $P_{0}=0, P_{1}=1$, and generalize these identities for many similar sequences. We prove that the sum of $N>1$ consecutive Pell numbers is a fixed integer multiple of another Pell number if and only if $4\mid N$. We consider the generalized Pell $(k,i)$-numbers defined by $p(n) :=\ 2p(n-1)+p(n-k-1) $ for $n\geq k+1$, with $p(0)=p(1)=\cdots =p(i)=0$ and $p(i+1)=\cdots = p(k)=1$ for $0\leq i\leq k-1$, and prove that the sum of $N=2k+2$ consecutive terms is a fixed integer multiple of another term in the sequence. We also prove that for the generalized Pell $(k,k-1)$-numbers such a relation does not exist when $N$ and $k$ are odd. We give analogous results for the Fibonacci and other related second-order recursive sequences.

==> epsfig.tex <==
%%
%% This is file `epsfig.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% epsfig.dtx  (with options: `package')
%% 
%% epsfig.dtx Copyright (C) 1994-1996 1999 Sebastian Rahtz
%%
%% This file is part of the Standard LaTeX `Graphics Bundle'.
%% It may be distributed under the terms of the LaTeX Project Public
%% License, as described in lppl.txt in the base LaTeX distribution.
%% Either version 1.3 or, at your option, any later version.
%%
\NeedsTeXFormat{LaTeX2e}[1994/06/01]
\ProvidesPackage{epsfig}
                  [1999/02/16 v1.7a (e)psfig emulation (SPQR)]
\DeclareOption*{\PassOptionsToPackage{\CurrentOption}{graphicx}}
\ProcessOptions
\RequirePackage{graphicx}
\def\psfig#1{%
 \let\Gin@ewidth\Gin@exclamation\let\Gin@eheight\Gin@ewidth
 \def\Gin@req@sizes{%
   \def\Gin@scalex{1}\let\Gin@scaley\Gin@exclamation
   \Gin@req@height\Gin@nat@height
   \Gin@req@width\Gin@nat@width}%
   \begingroup
    \let\Gfigname\relax
    \@tempswafalse
    \toks@{\Ginclude@graphics{\Gfigname}}%
    \setkeys{Gin}{#1}%
    \Gin@esetsize
    \ifx\Gfigname\relax\ErrorNoFile\else
      \the\toks@
    \fi
  \endgroup}
\define@key{Gin}{figure}{\def\Gfigname{#1}}
\define@key{Gin}{file}{\def\Gfigname{#1}}
\define@key{Gin}{prolog}{\typeout{epsfig: header files are not needed}}
\define@key{Gin}{silent}[]{}
\def\psdraft{\Gin@drafttrue}
\def\psfull{\Gin@draftfalse}
\def\pssilent{\typeout{epsfig option `silent' ignored}}
\def\psnoisy{\typeout{epsfig option `noisy' ignored}}
\let\epsfig\psfig
\def\psfigdriver#1{\makeatletter\input{#1.def}\makeatother}
\newdimen\epsfxsize
\newdimen\epsfysize
\epsfysize\z@
\epsfxsize\z@
\def\epsfsize#1#2{\epsfxsize}
\def\epsfbox{%
 \@ifnextchar[%
  {\Gin@bboxtrue\epsf@bb@box}%
  {\Gin@bboxfalse\epsf@box}%
}
\def\epsf@bb@box[#1#2]{%
  \expandafter\Gread@parse@bb#1#2 \\
  \epsf@box}
\def\epsf@box#1{%
 \bgroup
   \def\Gin@req@sizes{%
        \epsfxsize\epsfsize{\Gin@nat@width}{\Gin@nat@height}%
        \ifdim\epsfxsize=\z@
            \ifdim\epsfysize=\z@
                \Gin@req@height\Gin@nat@height
                \Gin@req@width\Gin@nat@width
            \else
                \let\Gin@scalex\Gin@exclamation
                \Gin@req@height\epsfysize
                \Gscale@div\Gin@scaley\Gin@req@height\Gin@nat@height
                \Gin@req@width\Gin@scaley\Gin@nat@width
            \fi
        \else
            \Gin@req@width\epsfxsize
            \Gscale@div\Gin@scalex\Gin@req@width\Gin@nat@width
            \ifdim\epsfysize=\z@
                \let\Gin@scaley\Gin@exclamation
                \Gin@req@height\Gin@scalex\Gin@nat@height
            \else
                \Gin@req@height\epsfysize
                \Gscale@div\Gin@scaley\Gin@req@height\Gin@nat@height
            \fi
        \fi
      }%
 \Ginclude@graphics{#1}%
 \egroup
 \epsfysize\z@
 \epsfxsize\z@
}
\let\epsffile\epsfbox
\def\epsfclipon{\Gin@cliptrue}
\def\epsfclipoff{\Gin@clipfalse}
\def\epsfverbosetrue{\typeout{epsf verbose option ignored}}
\def\epsfverbosefalse{\typeout{epsf verbose option ignored}}

\endinput
%%
%% End of file `epsfig.sty'.

